Driven damped harmonic oscillator revisited: energy resonance

We derive the exact expression for the resonant frequency of the time-averaged steady-state energy and show that this frequency is excellently approximated by the arithmetic mean of the amplitude and velocity resonant frequencies. In addition, we argue that the frequency of the amplitude resonance can be regarded as the energy resonance frequency, since it provides the maximal peak values of instantaneous energy.

==> Literature_examples.tex <==
@BOOK{Bire82,
   author       = {N. D. Birell and P. C. W. Davies},
   year         = 1982,
   title        = {Quantum Fields in Curved Space},
   publisher    = {Cambridge University Press}
}

@ARTICLE{feyn54,
   author       = "R. P. Feynman",
   year         = "1954",
   journal      = "Phys.\ Rev.",
   volume       = "94",
   pages        = "262",
}

@ARTICLE{epr,
   author       = "A. Einstein and {\relax Yu} Podolsky and N. Rosen", 
   year         = "1935", 
   journal      = "Phys.\ Rev.", 
   volume       = "47", 
   pages        = "777",
}

@ARTICLE{Berman1983,
   author       = "Berman, Jr., G. P. and Izrailev, Jr., F. M.",
   title        = "Stability of nonlinear modes",
   journal      = "Physica D",
   volume       = "88", 
   pages        = "445",
   year         = "1983",
}

@ARTICLE{Davies1998,
   author       = "E. B. Davies and L. Parns", 
   title        = "Trapped modes in acoustic waveguides", 
   journal      = "Q. J. Mech. Appl. Math.", 
   volume       = "51", 
   pages        = "477--492", 
   year         = "1988", 
}

@MISC{witten2001,
   author       = "Edward Witten",
   eprint       = "hep-th/0106109",
   year         = "2001", 
}

@INBOOK{Beutler1994,
   author       = "E. Beutler", 
   editor       = "E. Beutler and M. A. Lichtman and B. W. Coller and T. S. Kipps", 
   title        = "Williams Hematology", 
   chapter      = "7", 
   pages        = "654--662",
   publisher    = "McGraw-Hill", 
   year         = "1994", 
   edition      = "5", 
   address      = "New York", 
   volume       = "2", 
}

@INBOOK{inbook-full,
   author = "Donald E. Knuth",
   title = "Fundamental Algorithms",
   volume = 1,
   series = "The Art of Computer Programming",
   publisher = "Addison-Wesley",
   address = "Reading, Massachusetts",
   edition = "Second",
   month = "10~" # jan,
   year = "\noopsort{1973b}1973",
   type = "Section",
   chapter = "1.2",
   pages = "10--119",
   note = "A full INBOOK entry",
}

@ARTICLE{Smith2005,
   author       = "J. S. Smith and G. W. Johnson", 
   journal      = "Philos. Trans. R. Soc. London, Ser. B", 
   title        = "", 
   year         = "2005", 

   volume       = "777", 
   pages        = "1395",
}

@UNPUBLISHED{Smith2010,
   author       = "W. J. Smith and T. J. Johnson and B. G. Miller", 
   title        = "Surface chemistry and preferential crystal orientation on a silicon surface", 
   note         = "{J. Appl. Phys.} (unpublished)", 
   
   month        = "", 
   year         = "",
}

@UNPUBLISHED{Smith2010a,
   author       = "V. K. Smith and K. Johnson and M. O. Klein", 
   title        = "Surface chemistry and preferential crystal orientation on a silicon surface", 
   note         = "{J. Appl. Phys.} (submitted)", 
   
   month        = "", 
   year         = "",
}

@UNPUBLISHED{unpublished-full,
   author = "Ulrich {\"{U}}nderwood and Ned {\~N}et and Paul {\={P}}ot",
   title = "Lower Bounds for Wishful Research Results",
   month = nov # ", " # dec,
   year = 1988,
   note = "Talk at Fanstord University (A full UNPUBLISHED entry)",
}

@MISC{JohnsonMillerSmith2007, 

   author       = "M. P. Johnson and K. L. Miller and K. Smith", 
   title        = "", 
   howpublished = "personal communication", 
   month        = "1~" # may, 
   year         = "2007", 
   note         = "",
}

@PROCEEDINGS{Smith2007, 
   title        = "AIP Conf. Proc.", 
   year         = "2007", 
   
   editor       = "J. Smith", 
   volume       = "841", 
   number       = "21", 
   series       = "", 
   address      = "", 
   month        = "", 
   organization = "", 
   publisher    = "", 
   note         = "", 
}

@PROCEEDINGS{proceedings-full,
   editor = "Wizard V. Oz and Mihalis Yannakakis",
   title = "Proc. Fifteenth Annual",
   number = 17,
   series = "All ACM Conferences",
   month = mar,
   year = 1983,
   address = "Boston",
   organization = "ACM",
   publisher = "Academic Press",
   note = "A full PROCEEDINGS entry",
}

@UNPUBLISHED{Burstyn2004,
   author       = "Y. Burstyn", 
   title        = "{Proceedings of the 5th International Molecular Beam Epitaxy Conference, Santa Fe, NM}", 
   note         = "(unpublished)", 
   
   month        = "5--8~" # oct, 
   year         = "2004",
}

@PROCEEDINGS{Quinn2001, 
   title        = "{Proceedings of the 2003 Particle  Accelerator Conference, Portland, OR, 12-16 May 2005}", 
   year         = "2001", 
   
   editor       = "B. Quinn", 
   address      = "New York", 
   publisher    = "Wiley", 
   note         = "Albeit the conference was held in 2005, it was the 2003 conference, and  the proceedings were published in 2001; go figure", 
}

@ARTICLE{Agarwal2001,
   author       = "A. G. Agarwal", 
   title        = "{Proceedings of the Fifth Low Temperature Conference, Madison, WI, 1999}", 
   journal      = "Semiconductors", 
   year         = "2001", 

   volume       = "66", 
   pages        = "1238", 
}

@ARTICLE{SmithDA01,
   author       = "R. Smith",
   title        = "Hummingbirds are our friends",
   journal      = {J. Appl. Phys. (these proceedings)},
   year         = "",
   volume       = "",
   number       = "",
   pages        = "",
   month        = "",
   note         = "Abstract No. DA-01",
}

@ARTICLE{Smith2007a, 
   author       = "J. Smith", 
   title        = "", 
   journal      = "Proc. SPIE", 
   year         = "2007", 

   volume       = "124", 
   pages        = "367", 
   note         = "Required title is missing", 
}

@TECHREPORT{techreport-full,
   author = "Tom T{\'{e}}rrific",
   title = "An {$O(n \log n / \! \log\log n)$} Sorting Algorithm",
   institution = "Fanstord University",
   type = "Wishful Research Result",
   number = "7",
   address = "Computer Science Department, Fanstord, California",
   month = oct,
   year = 1988,
   note = "A full TECHREPORT entry",
}

@TECHREPORT{Nelson1999, 
   author       = "J. Nelson", 
   type         = "{TWI Report}", 
   number       = "666/1999",
   institution  = "", 
   year         = jan # "~1999", 
   
   note         = "Required institution missing", 
}

@TECHREPORT{Fields2005, 
   author       = "W. K. Fields", 
   type         = "{ECE Report No.}", 
   number       = "AL944",
   institution  = "", 
   year         = "2005", 
   
   note         = "Required institution missing", 
}

@MISC{Zalkins2008, 

   author       = "Y. M. Zalkins", 
   title        = "", 
   howpublished = "e-print arXiv:cond-mat/040426", 
   month        = "", 
   year         = "2008", 
   note         = "",
}

@MISC{Nelson2005, 

   author       = "J. Nelson", 
   howpublished = "{U.S. Patent No.} 5,693,000", 
   year         = "12~" # dec # "~2005", 
}

@MASTERSTHESIS{Nelson1999a,
   author       = "J. K. Nelson", 
   title        = "", 
   school       = "New York University", 
   year         = "1999", 
   
   type         = "M.{S}. thesis", 
   address      = "", 
   month        = "", 
   note         = "", 
}

@MASTERSTHESIS{mastersthesis-full,
   author = "{\'{E}}douard Masterly",
   title = "Mastering Thesis Writing",
   school = "Stanford University",
   type = "Master's project",
   address = "English Department",
   month = jun # "-" # aug,
   year = 1988,
   note = "A full MASTERSTHESIS entry",
}

@PHDTHESIS{Smith2003,
   author       = "S. M. Smith", 
   title        = "", 
   school       = "Massachusetts Institute of  Technology", 
   year         = "2003", 
   
   type         = "{Ph.D.} thesis", 
   address      = "", 
   month        = "", 
   note         = "", 
}

@ARTICLE{KawaLin2003,
   author       = "S. R. Kawa and S.-J. Lin", 
   title        = "", 
   journal      = "J. Geophys. Res.", 
   year         = "2003", 

   volume       = "108", 
   number       = "D6", 
   pages        = "4201", 
   month        = "", 
   note         = "{DOI:10.1029/2002JD002268}", 
}

@PHDTHESIS{phdthesis-full,
   author = "F. Phidias Phony-Baloney",
   title = "Fighting Fire with Fire: Festooning {F}rench Phrases",
   school = "Fanstord University",
   type = "{PhD} Dissertation",
   address = "Department of French",
   month = jun # "-" # aug,
   year = 1988,
   note = "A full PHDTHESIS entry",
}

@BOOK{book-full,
   author = "Donald E. Knuth",
   title = "Seminumerical Algorithms",
   volume = 2,
   series = "The Art of Computer Programming",
   publisher = "Addison-Wesley",
   address = "Reading, Massachusetts",
   edition = "Second",
   month = "10~" # jan,
   year = "\noopsort{1973c}1981",
   note = "A full BOOK entry",
}

@BOOKLET{booklet-full,
   author = "Jill C. Knvth",
   title = "The Programming of Computer Art",
   howpublished = "Vernier Art Center",
   address = "Stanford, California",
   month = feb,
   year = 1988,
   note = "A full BOOKLET entry",
}

@INBOOK{ballagh2000,
   author    = "R. Ballagh and C.M. Savage",
   editor    = "C.M. Savage and M. Das",
   title     = "Bose-Einstein condensation: from atomic physics to quantum fluids, Proceedings of the 13th Physics Summer School",
   year      = "2000",
   publisher = "World Scientific",
   address   = "Singapore",
   eprint    = "cond-mat/0008070",
}

@inBook{Magnetism,
   author    = "W. Opechowski and R. Guccione",
   title     = "Introduction to the Theory of Normal Metals",
   volume    = "IIa",
   pages     = "105",
   editor    = "G. T. Rado and H. Suhl",
   booktitle = "Magnetism",
   publisher = "Academic Press",
   address   = "New York",
}
   year      = "1965",

@INPROCEEDINGS{Magnetismb,
   author    = "W. Opechowski and R. Guccione",
   title     = "Introduction to the Theory of Normal Metals",
   editor    = "G. T. Rado and H. Suhl",
   booktitle = "Magnetism",
   volume    = "IIa",
   pages     = "105",
   publisher = "Academic Press",
   address   = "New York",
   year      = "1965",
}

@INBOOK{Smith80,
   author    = "J. M. Smith",
   title     = "Molecular Dynamics",
   publisher = "Academic",
   year      = "1980",
   address   = "New York",
   editor    = "C. Brown",
}

@article{ZS71,
   author       = "V. E. Zakharov and A. B. Shabat",
   year         = "1971",
   title        = "Exact theory of two-dimensional self-focusing and one-dimensional self-modulation of waves in nonlinear media",
   journal      = "Zh. Eksp. Teor. Fiz.",
   volume       = "61",
   pages        = "118--134",
   translation  = "Sov. Phys. JETP \textbf{34}, 62 (1972)"
}

@INCOLLECTION{Beutler1994a,
   author       = "E. Beutler", 
   year         = "1994", 
   booktitle    = "Williams Hematology", 
   edition      = "5", 
   chapter      = "7", 
   editor       = "E. Beutler and M. A. Lichtman and B. W. Coller and T. S. Kipps", 
   publisher    = "McGraw-Hill", 
   address      = "New York", 
   volume       = "2", 
   pages        = "654--662",
}

@INCOLLECTION{ballagh2000a,
   author       = "R. Ballagh and C.M. Savage",
   year         = "2000",
   title        = "Bose-Einstein condensation: from atomic physics to quantum fluids",
   booktitle    = "Proceedings of the 13th Physics Summer School",
   editor       = "C.M. Savage and M. Das",
   publisher    = "World Scientific",
   address      = "Singapore",
   eprint       = "cond-mat/0008070",
}

@INCOLLECTION{Magnetisma,
   author       = "W. Opechowski and R. Guccione",
   year         = "1965",
   title        = "Introduction to the Theory of Normal Metals",
   booktitle    = "Magnetism",
   editor       = "G. T. Rado and H. Suhl",
   publisher    = "Academic Press",
   address      = "New York",
   volume       = "IIa",
   pages        = "105",
}

@INCOLLECTION{Smith80a,
   author       = "J. M. Smith",
   year         = "1980",
   booktitle    = "Molecular Dynamics",
   editor       = "C. Brown",
   publisher    = "Academic",
   address      = "New York",
}

@INCOLLECTION{incollection-full,
   key          = "incol-ful",
   author       = "Daniel D. Lincoll",
   year         = 1977,
   title        = "Semigroups of Recurrences",
   booktitle    = "High Speed Computer and Algorithm Organization",
   edition      = "Third",
   series       = "Fast Computers",
   number       = 23,
   chapter      = 3,
   type         = "Part",
   editor       = "David J. Lipcoll and D. H. Lawrie and A. H. Sameh",
   publisher    = "Academic Press",
   address      = "New York",
   month        = sep,
   pages        = "179--183",
   note         = "A full INCOLLECTION entry",
}

@INPROCEEDINGS{inproceedings-full,
   author = "Alfred V. Oaho and Jeffrey D. Ullman and Mihalis Yannakakis",
   title = "On Notions of Information Transfer in {VLSI} Circuits",
   editor = "Wizard V. Oz and Mihalis Yannakakis",
   booktitle = "Proc. Fifteenth Annual ACM",
   number = 17,
   series = "All ACM Conferences",
   pages = "133--139",
   month = mar,
   year = 1983,
   address = "Boston",
   organization = "ACM",
   publisher = "Academic Press",
   note = "A full INPROCEDINGS entry",
}

@MANUAL{manual-full,
   author = "Larry Manmaker",
   title = "The Definitive Computer Manual",
   organization = "Chips-R-Us",
   address = "Silicon Valley",
   edition = "Silver",
   month = apr # "-" # may,
   year = 1986,
   note = "A full MANUAL entry",
}
